Convergence of Recursive Stochastic Algorithms using Wasserstein Divergence

This paper develops a unified framework, based on iterated random operator theory, to analyze the convergence of constant stepsize recursive stochastic algorithms (RSAs). RSAs use randomization to efficiently compute expectations, and so their iterates form a stochastic process. The key idea of our analysis is to lift the RSA into an appropriate higher-dimensional space and then express it as an equivalent Markov chain. Instead of determining the convergence of this Markov chain (which may not converge under constant stepsize), we study the convergence of the distribution of this Markov chain. To study this, we define a new notion of Wasserstein divergence. We show that if the distribution of the iterates in the Markov chain satisfy a contraction property with respect to the Wasserstein divergence, then the Markov chain admits an invariant distribution. We show that convergence of a large family of constant stepsize RSAs can be understood using this framework, and we provide several detailed examples.

==> 7-applications.tex <==
We first consider a portfolio optimization problem over time horizon $t = 0, 1, \ldots, T$. There is a riskless asset with price $B_t$ (bond investment) that evolves according to
$$
B_{t+1} = (1 + r_t) B_t.
$$
There are also $M$ risky assets with price vector $S_t = (S_t^1,\ldots,\, S_t^M)$ (stock investments) with prices that evolve according to
$$
S_{t+1}^m = S_t^m \xi_{t+1}^m,
$$
where $\xi_t = (\xi_t^1, \ldots, \xi_t^M)$ are independent (so $S_t$ is Markov).

A portfolio strategy is a process $x_t = (x_t^0, x_t^1,\ldots, x_t^M)$ where $x_t^0$ is the number of units of the riskless asset and $x_t^m$ is the number of units of risky asset $m$. The value of the portfolio at time $t$ is then
$$
V_t = B_t x_t^0 + \sum_{m=1}^M S_t^m x_t^m.
$$
A portfolio is said to be self-financing if
$$
B_t x_t^0 + \sum_{m=1}^M S_t^m x_t^m = B_t x_{t+1}^0 + \sum_{m=1}^M S_t^m x_{t+1}^m.
$$
We are concerned with maximizing expected utility of terminal wealth:
$$
\max_{x} \left\{ \mathbb{E} [u(V_T^x)] : x \textrm{ self-financing} \right\}.
$$

The dynamic programming equations for the portfolio optimization problem are as follows. By the self-financing property, the portfolio value evolves according to:
$$
V_{t+1}(x_t,\, \xi_{t+1}) = V_t + V_t \left[ x_t^0 r_t + \sum_{m=1}^M x_t^m(\xi_{t+1}^m - 1) \right].
$$
Then, the DP recursion is $U_T(v) = u(v)$ and
$$
U_t(v) = \max_{x_t} \mathbb E[U_{t+1}(V_{t+1}(x_t,\, \xi_{t+1}))\, \vert \, V_t = v],
$$
for all $t = 1,\ldots,\,T-1$. The utility-to-go problem above has the implicit constraint
$$
v = B_t x_{t+1}^0 + \sum_{m=1}^M S_t^m x_{t+1}^m,
$$
given current portfolio value $v$.
